Simple Heuristics Yield Provable Algorithms for Masked Low-Rank Approximation

In $masked\ low-rank\ approximation$, one is given $A \in \mathbb{R}^{n \times n}$ and binary mask matrix $W \in \{0,1\}^{n \times n}$. The goal is to find a rank-$k$ matrix $L$ for which: $$cost(L) = \sum_{i=1}^{n} \sum_{j = 1}^{n} W_{i,j} \cdot (A_{i,j} - L_{i,j} )^2 \leq OPT + \epsilon \|A\|_F^2 ,$$ where $OPT = \min_{rank-k\ \hat{L}} cost(\hat L)$ and $\epsilon$ is a given error parameter. Depending on the choice of $W$, this problem captures factor analysis, low-rank plus diagonal decomposition, robust PCA, low-rank matrix completion, low-rank plus block matrix approximation, and many problems. Many of these problems are NP-hard, and while some algorithms with provable guarantees are known, they either 1) run in time $n^{\Omega(k^2/\epsilon)}$ or 2) make strong assumptions, e.g., that $A$ is incoherent or that $W$ is random. In this work, we show that a common polynomial time heuristic, which simply sets $A$ to $0$ where $W$ is $0$, and then finds a standard low-rank approximation, yields bicriteria approximation guarantees for this problem. In particular, for rank $k' > k$ depending on the $public\ coin\ partition\ number$ of $W$, the heuristic outputs rank-$k'$ $L$ with cost$(L) \leq OPT + \epsilon \|A\|_F^2$. This partition number is in turn bounded by the $randomized\ communication\ complexity$ of $W$, when interpreted as a two-player communication matrix. For many important examples of masked low-rank approximation, including all those listed above, this result yields bicriteria approximation guarantees with $k' = k \cdot poly(\log n/\epsilon)$. Further, we show that different models of communication yield algorithms for natural variants of masked low-rank approximation. For example, multi-player number-in-hand communication complexity connects to masked tensor decomposition and non-deterministic communication complexity to masked Boolean low-rank factorization.

==> fpt.tex <==
% !TEX root = factor_analysis.tex

\section{Fixed-Parameter-Tractable Algorithms via Communicatiom Complexity}\label{sec:fpt}

We conclude by discussing how communication complexity can be used to give fixed-parameter tractable algorithms  for Problem \ref{def:main}. While significantly less efficient then the polynomial time bicriteria approximation algorithms of Theorems \ref{thm:1} and \ref{thm:2}, these methods output $L$ with rank exactly $k$ -- without requiring bicriteria approximation. By the lower bound given in \cite{razenshteyn2016weighted} achieving this error with rank-$k$ is not possible in general in polynomial time under a variant of ETH.

In the case that the weight matrix $W$ is $0$ on its diagonal and $1$ off the diagonal, corresponding to the low-rank plus diagonal (LRPD) approximation problem, 
%which we give a $O(k/\epsilon)$ bicriteria approximation for in Cor. \ref{cor:lrpd}), 
the results of this section can be strengthened further to obtain a relative error approximation. See Appendix \ref{app:alt}. Interestingly, the main structural result used to obtain this approximation can also be used to give an alterative proof of our bicriteria bounds for the low-rank plus diagonal and low-rank plus sparse matrix approximation problems -- Cors. \ref{cor:lrpd} and \ref{cor:lrps}.

Our results in this section will critically rely on a result given in \cite{razenshteyn2016weighted} for a generalization of Problem \ref{def:main} where $W$ can be any positive weight matrix.
\begin{theorem}[Theorem 1.1 of \cite{razenshteyn2016weighted}]\label{thm:weighted1}
Given $W \in \R_{\ge 0}^{n \times n}$ with rank $r$ there is an algorithm running in $n^{O(k^2 r/\epsilon)}$ time that outputs with probability $\ge 9/10$ rank-$k$ $L$ satisfying:
\begin{align*}
\norm{W \circ (A -L)}_F^2 \le (1+\epsilon) OPT
\end{align*}
where $\displaystyle OPT = \min_{\rank-k\ \hat L} \norm{W \circ (A -\hat L)}_F^2$.
\end{theorem}

%\begin{theorem}[Theorem 1.2 of \cite{razenshteyn2016weighted}]\label{thm:weighted2}
%Given $n \times n$ weight matrix $W$ containing $r$ distinct columns, there is an algorithm running in $O((\nnz(A) + \nnz(W)) \cdot n^\gamma) + n\cdot 2^{\tilde O(k^2 r^2/\epsilon)}$ time for any $\gamma > 0$ that outputs with probability $\ge 9/10$ rank-$k$ $L$ satisfying:
%\begin{align*}
%\norm{W \circ (A -L)}_F^2 \le (1+\epsilon) OPT
%\end{align*}
%where $\displaystyle OPT = \min_{\rank-k\ \hat L} \norm{W \circ (A -\hat L)}_F^2$.
%\end{theorem}

We can bound the rank of (a close approximation to) $W$ using the randomized communication complexity, allowing us to apply the algorithms of \cite{razenshteyn2016weighted}. To bound the error incurred from using an approximation to $W$ given by a communication protocol, we will consider a slight modification of Problem \ref{def:main} in which the cost function is `regularized' by $\norm{L}_F^2$. I.e., we seek $L$ approximately solving
\begin{align*}
\min_{\rank-k\ \hat L} \norm{W \circ (A -\hat L)}_F^2 + \lambda \norm{L}_F^2
\end{align*}

\begin{theorem}[Randomized Communication Complexity $\rightarrow$ FPT Algorithm]\label{thm:OurWeighted1} Consider $W \in \{0,1\}^{n \times n}$ and let $f$ be the function computed by it. There is an algorithm that with probability $\ge 4/5$ outputs rank-$k$ $L$ satisfying:
\begin{align*}
\norm{W \circ (A -L)}_F^2 \le (1+\epsilon) OPT + \frac{\epsilon}{\lambda} \norm{A}_F^2 %+ \epsilon_2 \norm{L_{opt}}_F^2
\end{align*}
where $\displaystyle OPT = \min_{\rank-k\ \hat L} \norm{W \circ (A -\hat L)}_F^2 + \lambda \norm{\hat L}_F^2$.% and $L_{opt}$ is any rank-$k$ matrix achieving $OPT$. 
The algorithm runs in time $n^{O\left (\frac{k^2}{\epsilon} \cdot 2^{R_{\epsilon}^{1-sided}(\neg f)}\right )} + O(n \cdot 2^{R_{\epsilon}^{1-sided}(\neg f)} \cdot T)$, where $T$ is the total
time complexity to run a protocol achieving $R_{\epsilon}^{1-sided}(\neg f)$,
\end{theorem}
\begin{proof}
%$R_{\epsilon_1,\epsilon_2}(f)$ is the minimum number so that there is a distribution on protocols inducing partitions of $W$, each containing at most $2^{R_{\epsilon_1,\epsilon_2}(f)}$ rectangles, such that (1) for every $x,y \in \{0,1\}^{\log  n}$ with $f(x,y) = 1$, $(x,y)$ lands in a rectangle labeled $1$ with probability $\ge 1- \epsilon_1$ and (2) for every $x,y \in \{0,1\}^{\log  n}$ with $f(x,y) = 0$, $(x,y)$ lands in a rectangle  labeled $0$ with probability $\ge 1-\epsilon_2$. 
As discussed in the proof of Theorem \ref{thm:rand}, letting $W_\Pi$ be the (random) matrix corresponding to the function computed by a protocol achieving $R_{\epsilon}^{1-sided}(\neg f)$, $W \circ (1-W_\Pi)$ has each entry equal to $1$ with probability at most $\epsilon$ and $W_\Pi \circ (1-W) = 0$, since the protocol never errs where $W = 0$ (i.e., where $\neg f = 1$). Further $W_\Pi$ can be tiled by $2^{R_{\epsilon}^{1-sided}(\neg f)}$ monochromatic rectangles and so it is well known that $\rank(W_\Pi) \le 2^{R_{\epsilon}^{1-sided}(\neg f)}.$
We have:
\begin{align*}
\E_{protocol\ \Pi} \left [\norm{A \circ W \circ (1-W_\Pi)}_F^2 \right ] %+ \norm{L_{opt} \circ W_\Pi \circ (1-W)}_F^2\right ] 
\le \epsilon \norm{A \circ W}_F^2 %+ \epsilon_2 \norm{L_{opt} \circ (1- W)}_F^2\\
\le \epsilon \norm{A}_F^2.% + \epsilon_2 \norm{L_{opt}}_F^2.% \\ &\le \epsilon_1 \norm{A}_F^2 + \epsilon_2 \left (\norm{A - L_{opt} \circ W}_F^2 \right )\\
%&\le (\epsilon_1 +\epsilon_2) \norm{A}_F^2 + \epsilon_2 \norm{L_{opt}}_F^2.
\end{align*}
%The second inequality follows from the fact that if we had $\norm{L_{opt}}_F^2 \ge \norm{A - A \circ W}_F^2$ BLAH
Thus by Markov's inequality, with probability at least $9/10$, a randomly selected protocol satisfies:
\begin{align}\label{eq:plowF}\norm{A \circ W \circ (1-W_\Pi)}_F^2 \le 10 \epsilon \norm{A}_F^2.%+ \norm{L_{opt} \circ W_\Pi \circ (1-W)}_F^2 \le 10\epsilon_1 \norm{A}_F^2 + 10\epsilon_2 \norm{L_{opt}}_F^2 .
\end{align}
By Lemma \ref{lem:compProt} we can compute such a $W_{\Pi}$ with probability $9/10$ in $n \cdot 2^{|\Pi|} \cdot T$ where $T$ is the total
time complexity of the players to run the protocol. We simple sample a random protocol, and then use Lemma \ref{lem:compProt} to compute a representation of $W_\Pi$ in terms of its rectangles. Once we have computed $W_\Pi$, we will apply Theorem \ref{thm:weighted1}, to compute with probability $\ge 9/10$, $\bar L$ satisfying:
\begin{align}\label{eq:minReg}
\norm{W_\Pi \circ (A-\bar L)}_F^2 \le (1 + \epsilon) \cdot \min_{\rank-k\ \hat L} \norm{(W_\Pi + \gamma 1) \circ (A-\hat L)}_F^2.
\end{align}
Note that we have `regularized' $W$ by adding a weighted copy of the all ones matrix for weight $\gamma$ that we will set later. This increases the rank of $W$ by at most $1$ and so the runtime is still $n^{O\left (\frac{k^2}{\epsilon} \cdot \rank(W_\Pi)\right )} \le n^{O\left (\frac{k^2}{\epsilon} \cdot 2^{R_{\epsilon_1,\epsilon_2}(f)}\right )}$. Giving the claimed total runtime and success probability $\ge 8/10$ via a union bound over the success of Theorem \ref{thm:weighted1} and the bound of \eqref{eq:plowF} holding. 

We now analyze the error of $\bar L$. Note that for appropriately set $\lambda$, since we can always scale the weight matrix without changing the minimization problem of \eqref{eq:minReg}, this problem is identical minimizing $\norm{[W_\Pi + \sqrt{\lambda} (I-W_\Pi)] \circ (A-\hat L)}_F^2 = \norm{W_\Pi \circ (A - \hat L)}_F^2 + \lambda \norm{(I-W_\Pi) \circ \hat L}_F^2.$ We have:

%\begin{align*}
%\norm{ (A - \bar L)\circ W}_F^2 &= \norm{ (A - \bar L)\circ W_\Pi}_F^2 + \norm{ (A - \bar L)\circ W \circ (1-W_\Pi)}_F^2\\
%&\le \norm{ (A - \bar L)\circ W_\Pi \circ W}_F^2
%\end{align*}
\begin{align*}
\norm{ (A - \bar L)\circ W}_F^2 &= \norm{(A - \bar L) \circ W_\Pi \circ W}_F^2 +  \norm{(A - \bar L) \circ (1-W_\Pi) \circ W}_F^2\\
&\le  \norm{(A - \bar L) \circ W_\Pi}_F^2 +  \norm{(A - \bar L) \circ (1-W_\Pi)}_F^2
%&\le  (1+\epsilon) \norm{(A - \hat L) \circ W_\Pi}_F^2 +  0\\
%&\le  (1+\epsilon) \norm{(A - L_{opt}) \circ W_\Pi \circ W}_F^2 +  (1+\epsilon) \norm{(A - L_{opt}) \circ W_\Pi \circ (1-W)}_F^2  + \norm{(A - \bar L) \circ (1-W_\Pi) \circ W}_F^2\\
%&\le (1+\epsilon) OPT + 0
\end{align*}
\end{proof}

==> one_way.tex <==
% !TEX root = factor_analysis.tex

\section{Column Subset Selection via One-Way Communication Complexity}

In this section we use one-way communication complexity to give an approximation result for masked column subset selection (also known as column-based matrix approximation). In column subset selection, one seeks to identify a small subset of columns of $A$ whose span contains a good approximation to the matrix \cite{deshpande2010efficient,guruswami2012optimal,boutsidis2014near}. Since the left factor of the low-rank approximation is itself a subset of actual columns of $A$, such an approximation can preserve sparsity, interpretability, and other properties. We refer the reader to the surveys for more discussion of this widely studied primitive \cite{m11,w14}.

In the {\it masked column subset selection} problem, one is given $A \in \mathbb{R}^{n \times n}$ and a weight matrix $W \in \{0,1\}^{n \times n}$ and seeks to find a subset $C \in \R^{n \times k}$ of at most $k$ columns of $A$ minimizing:
\begin{eqnarray*}
\textrm{cost}(C) = \min_{X \in \mathbb{R}^{n \times k}} \|W \circ (C \cdot X^T - A)\|_F^2. %\leq OPT + \epsilon \|A\|_F^2,
\end{eqnarray*}
Even in the non-masked setting, finding an optimal $C$ for a given rank $k$ is NP-Hard \cite{ccivril2014column,shitov2017column}. Thus, most results on column subset selection in the unmasked setting consider bicriteria approximation guarantees, showing how to find a subset of $k'$ columns with reconstruction cost nearly as small as the cost of the best (un-constrained) rank-$k$ approximation to $A$ \cite{deshpande2010efficient,guruswami2012optimal,m11,w14}. We give an analogous bound in the masked setting in terms of the 1-way communication complexity of $W$.
%where $OPT = \min_{\rank-k\ \hat L} \norm{(A-\hat L)\circ W}_\star$ is the cost of the best masked rank-$k$ approximation of $A$.
For simplicity, we give the bound for the squared Frobenius norm, however an analogous bound can be given for any entrywise norm that admits an efficient non-masked column subset selection algorithm.


\begin{theorem}[One Way Communication Complexity $\rightarrow$ Column Subset Selection]\label{thm:row}
Consider $W \in \{0,1\}^{n \times n}$ and let $f$ be the function computed by it. Let $k' =  2k/\epsilon_3 \cdot 2^{R_{\epsilon_1,\epsilon_2}^{1-way}(f)}$.%, where $k_\star$ is the smallest integer such that for any $M \in \R^{n \times n}$, there exists $C$ with $k_\star$ columns and $X \in n \times k_\star$ satisfying $\displaystyle \norm{M-C \cdot X^T}_{\star} \le \min_{\rank-k\ L}\norm{M-L}_\star$. 
There is an algorithm running in $\tilde O\left (\nnz(A) + 2^{R_{\epsilon_1,\epsilon_2}^{1-way}(f)}\cdot n \cdot (T + \poly(k/\epsilon))\right )$ time and outputing $C,X \in \R^{n \times k'}$ satisfying with high probability:
\begin{align*}
\norm{(A-C\cdot X^T) \circ W}_F^2 \le OPT + (2\epsilon_1+\epsilon_3) \norm{A \circ W}_F^2 + 2\epsilon_2 \norm{L_{opt} \circ (1-W)}_F^2,
\end{align*}
where $L_{opt} = \argmin_{\rank-k\ L} \norm{(A-L)\circ W}_F^2$, $OPT =  \norm{(A-L_{opt})\circ W}_F^2$, and $T$ is the time complexity to run a protocol for $f$ achieving ${R_{\epsilon_1,\epsilon_2}^{1-way}(f)}$.
\end{theorem}
\begin{proof}
As discussed in Definition \ref{def:1way}, $R^{1-way}_{\epsilon_1,\epsilon_2}(f)$ is the minimum number so that there is a distribution on protocols corresponding to partitions of $W$ such that (1) for each partition of $W$, there is some partition $P_C$ of the columns of $W$ with $|P_C| \le R^{1-way}_{\epsilon_1,\epsilon_2}(f)$ such that all rectangles in the partition are of the form $R = r \times c$ where $c \in P_C$ and $r \subseteq \{0,1\}^{\log n}$ and (2) for every $(x,y) \in \mathcal{X} \times \mathcal{Y}$ with $f(x,y) = 1$, with probability at least $1-\epsilon_1$, $(x,y)$ lands in a rectangle which is labeled $1$ and for every $(x,y) \in \mathcal{X} \times \mathcal{Y}$ with $f(x,y) = 0$, with probability at least $1-\epsilon_2$, $(x,y)$ lands in a rectangle which is labeled $0$.

Following the proof of Theorem \ref{thm:rand}, letting $W_\Pi$ be the (random) matrix corresponding to the function computed by the protocol. We have:
\begin{align*}
\E_{protocol\ \Pi} \left [\norm{A \circ W \circ (1-W_\Pi)}_F^2 + \norm{L_{opt} \circ W_\Pi \circ (1-W)}_F^2\right ] &\le \epsilon_1 \norm{A \circ W}_F^2 + \epsilon_2 \norm{L_{opt} \circ (1- W)}_F^2.
%&\le \epsilon_1 \norm{A}_\star + \epsilon_2 \norm{L_{opt}}_\star.% \\ &\le \epsilon_1 \norm{A}_\star + \epsilon_2 \left (\norm{A - L_{opt} \circ W}_\star \right )\\
%&\le (\epsilon_1 +\epsilon_2) \norm{A}_\star + \epsilon_2 \norm{L_{opt}}_\star.
\end{align*}
Thus choosing a random protocol $\Pi$, by Markov's inequality, with probability at least $1/2$ we have: 
\begin{align}\label{eq:plow2}\norm{A \circ W \circ (1-W_\Pi)}_F^2 + \norm{L_{opt} \circ W_\Pi \circ (1-W)}_F^2 \le 2\epsilon_1 \norm{A \circ W }_F^2 + 2\epsilon_2 \norm{L_{opt} \circ (1-W)}_F^2 .
\end{align}
Consider a protocol satisfying \eqref{eq:plow2} and let $P_C$ be its corresponding column partition, consisting of at most $2^{R_{\epsilon_1,\epsilon_2}^{1-way}(f)}$ sets. For each set of columns $R_i \in P_C$ let $R_{i,1}$ be the rectangle on those columns labeled $1$. Let $C_i$ be a subset of  $2k/\epsilon_3$ columns of $R_i$ and $C_{i,1}$ be the rows of that subset intersecting $R_{i,1}$. Let $X_i$ be a $|R_i| \times 2k/\epsilon_3$  matrix such that:
\begin{align}\label{css}
\norm{C_{i,1} \cdot X_i^T -R_{i,1}}_F^2 \le (1+\epsilon_3) \min_{\rank-k\ L} \norm{R_{i,1} - L}_F^2.
\end{align}
It is well known that for any matrix $R_{i,1}$, such a column subset with $2k/\epsilon_3$ columns satisfying \eqref{css} exists \cite{guruswami2012optimal}. Further $C_i$ and $X_i$ can be bound in $O(\nnz(R_i) + n \cdot \poly(k/\epsilon))$ time. We can explicitly construct the partition $P_C$ and find a column subset for each $R_i \in P_C$ in total time  $O\left (\nnz(A) + 2^{R_{\epsilon_1,\epsilon_2}^{1-way}(f)}\cdot n \cdot (T + \poly(k/\epsilon))\right )$.

Let $C = \cup_{R_i \in P_C} C_i$. That is, $C$ is the union of the good column subsets for each $R_i$. Note that $| C| = 2k/\epsilon_3 \cdot 2^{R_{\epsilon_1,\epsilon_2}^{1-way}(f)} = k'$. Let $X \in \R^{n \times k'}$ be the block diagonal matrix obtained by appending each $X_i$ in the natural way so that $C X^T = [C_1 X_1^T, \ldots,  C_{|P_C|} X_{|P_C|}^T].$
We can bound:
\begin{align*}
\norm{(A - C  X^T) \circ W}_F^2 %&= \norm{(A \circ W - C  X^T \circ W}_F^2\\
&= \norm{(A - C  X^T) \circ W \circ W_\Pi}_F^2 + \norm{(A - C  X^T) \circ W \circ (1-W_\Pi)}_F^2\\
%&\le  \norm{(A - C  X^T) \circ W_\Pi}_F^2 + \norm{(A - C  X^T) \circ (1-W_\Pi)}_F^2\\
%&= \sum_{R_i \in P_C} \norm{R_{i,1} - C_{i,1} X_i^T}_F^2 + BLAH\\
%&\le (1+\epsilon_3) \min_{\rank-k\ L} \norm{(A - L) \circ W_\Pi}_F^2
\end{align*}
The first term can be bounded as
\begin{align*}
 \norm{(A - C  X^T) \circ W \circ W_\Pi}_F^2 &\le  \norm{(A - C  X^T) \circ W_\Pi}_F^2\\
 &= \sum_{R_i \in P_C} \norm{R_{i,1} - C_{i,1} X_i^T}_F^2\\
  &\le (1+\epsilon_3) \sum_{R_i \in P_C} \min_{\rank-k\ L} \norm{R_{i,1} - L}_F^2\\
 &\le (1+\epsilon_3) \min_{\rank-k\ L} \norm{(A - L) \circ W_\Pi}_F^2\\
 &\le (1+\epsilon_3) \min_{\rank-k\ L} \norm{(A - L) \circ W}_F^2 = (1+\epsilon_3) OPT
\end{align*} 
where the line follows from the fact that the communication protocol has one sided error so the ones in $W_\Pi$ are a subset of those in $W$. The second term can be bounded as
\begin{align*}
\norm{(A - C  X^T) \circ W \circ (1-W_\Pi)}_F^2 \le BLAH
\end{align*}


By the assumption that $S, U$ satisfy $\norm{A\circ W - [A\circ W](S) \cdot U}_F^2 \le \min_{\hat S,\hat U} \norm{A\circ W - [A\circ W](\hat S) \cdot \hat U}_F^2 +\epsilon_3 \norm{A}_F^2$:
\begin{align*}
\norm{(A - [A\circ W](S) \cdot U) \circ W}_F^2 \le \norm{A \circ W - [A\circ W](S) \cdot U}_F^2 &\le \norm{A \circ W - [A\circ W](\bar S) \cdot \bar U}_F^2 + \epsilon_3 \norm{A}_F^2%\\
%&= \norm{(A \circ W - A(\bar S) \cdot \bar U) \circ (W_\Pi) }_\star +  \norm{(A \circ W - A(\bar S) \cdot \bar U) \circ (1-W_\Pi) }_\star \epsilon_3 \norm{A}_\star
\end{align*}
We now consider $ \norm{A \circ W - [A\circ W](\bar S) \cdot \bar U}_F^2 $. We can write:
\begin{align*}
\norm{A \circ W - [A\circ W](\bar S) \cdot \bar U}_F^2 &= \norm{[A \circ W - [A\circ W](\bar S) \cdot \bar U] \circ W_\Pi}_F^2 +  \norm{[A \circ W - [A\circ W](\bar S) \cdot \bar U] \circ (1-W_\Pi)}_F^2\\
&\le \norm{[A \circ W - [A\circ W](\bar S) \cdot \bar U] \circ W_\Pi}_F^2 + \norm{A \circ W \circ (1-W_\Pi)}_F^2
\end{align*}
where the inequality  follows from the fact that $\bar U$ projects each column of $A \circ W$ to the span of $[A \circ W](\bar S)$ and thus the error is at most the original norm.
Considering the first term we have:8
\begin{align*}
\norm{[A \circ W - [A\circ W](\bar S) \cdot \bar U] \circ W_\Pi}_F^2 \le BLAH
\end{align*}

Let $P_1 \subset P$ be the set  of rectangles on which the protocol returns $1$ and $P_0$ be the set where it returns $0$.
 For any $R \in P_1$ let $L_R = \argmin_{\rank-k\ L} \norm{A_R \circ W_R - L}_\star$. Let $\hat L_R$ be equal to $L_R$ on $R$ and $0$ elsewhere. Let 
$\hat L = \sum_{R \in P} (A_R)_k$. Note that $\hat L$ has rank at most $k \cdot 2^{R_{\epsilon_1, \epsilon_2}(f)}$. Thus we have by our assumption that $L$ satisfies $\norm{A \circ W - L}_\star \le \min_{rank-k'\ \hat L} \norm{A \circ W - \hat L}_\star + \epsilon_3 \norm{A}_\star$: 
\end{proof}

\subsection{Applications of Column-Based Approximation Theorem}

